A Comparison of Full-Scale Experimental Measurements and Computational Predictions of the Transom-Stern Wave of the R/V Athena I

Full-scale experimental measurements and numerical predictions of the wave-elevation topology behind a transom-sterned vessel, the R/V Athena I, are compared and assessed in this paper. The mean height, surface roughness (RMS), and spectra of the breaking stern-waves were measured in-situ by a LIDAR sensor over a range of ship speeds covering both wet- and dry-transom operating conditions. Numerical predictions for this data set from two Office of Naval Research (ONR) supported naval-design codes, NFA and CFDship-Iowa-V.4, have been performed. Initial comparisons of the LIDAR data to the numerical predictions at 5.4 m/s (10.5 kts), a wet-transom condition, are presented. This work represents an ongoing effort on behalf of the ONR Ship Wave Breaking and Bubble Wake program, to assess, validate, and improve the capability of Computational Fluid Dynamics (CFD) to predict full-scale ship-generated wave fields.

==> CFDShip/tables.tex <==
%\setlength{\paperwidth}{612pt}
%\setlength{\paperheight}{792pt}
%\setlength{\textheight}{648pt}
%\setlength{\textwidth}{432pt}
%\setlength{\voffset}{-72pt}
%\setlength{\hoffset}{-72pt}
%\setlength{\evensidemargin}{90pt}
%\setlength{\oddsidemargin}{90pt}
%\setlength{\topmargin}{39pt}
%\setlength{\headheight}{13pt}
%\setlength{\headsep}{20pt}

%\makeatletter
%	\newenvironment{indentation}[3]%
%	{\par\setlength{\parindent}{#3}
%	\setlength{\leftmargin}{#1}       \setlength{\rightmargin}{#2}%
%	\advance\linewidth -\leftmargin       \advance\linewidth -\rightmargin%
%	\parshape 1\@totalleftmargin \linewidth\ignorespaces}{\par}%
%\makeatother

% new LaTeX commands
\newcommand{\styleListParagraph}[1]{#1}


\begin{table}
\begin{center}
\vspace{3pt} \noindent
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 \parbox{54pt}{\raggedright\styleListParagraph{Simulations}} &
 \parbox{40pt}{\raggedright\styleListParagraph{Re}} &
 \parbox{17pt}{\raggedright\styleListParagraph{Fr}} &
 \parbox{32pt}{\raggedright\styleListParagraph{Time step $\Delta{}$t}} &
 \parbox{106pt}{\raggedright\styleListParagraph{Turbulence models}} &
 \parbox{47pt}{\raggedright\styleListParagraph{Motions}} \\
\hline
 \parbox{54pt}{\raggedright\styleListParagraph{Model-scale}} &
 \parbox{40pt}{\raggedright\styleListParagraph{11.5$\times{}$10$^{6}$}} &
 \parbox{17pt}{\raggedright\multirow{2}{*}\styleListParagraph{0.25}} &
 \parbox{32pt}{\raggedright\multirow{2}{*}\styleListParagraph{0.001}} &
 \parbox{106pt}{\raggedright\styleListParagraph{Blended k-$\epsilon{}$/k- based DES}} &
 \parbox{47pt}{\raggedright\multirow{2}{*}\styleListParagraph{Fixed sinkage and trim}} \\
\cline{1-2} \cline{5-5}
 \parbox{54pt}{\raggedright\styleListParagraph{Full-scale}} &
 \parbox{40pt}{\raggedright\styleListParagraph{2.9$\times{}$10$^{8}$}} &
 &
 &
 \parbox{106pt}{\raggedright\styleListParagraph{Blended k-/k- based DES with a multi-layer wall function (y$_{2}$$^{+ }$\textasciitilde{}100)}} &
 \\
\hline
\end{tabular}
\end{center}
\vspace{2pt}
\caption {\label{tab:????1}????1}
\end{table}


\begin{table}
\begin{center}
\vspace{3pt} \noindent
\begin{tabular}{|p{21pt}|p{72pt}|p{60pt}|p{36pt}|p{1pt}|p{1pt}|p{4pt}|p{28pt}|p{35pt}|p{39pt}|}
\hline
 \parbox{21pt}{\raggedright\multirow{2}{*}(\footnotesize Block }} &
 \parbox{72pt}{\raggedright\multirow{2}{*}{\footnotesize Name}} &
 \parbox{60pt}{\raggedright\multirow{2}{*}{\footnotesize Grid Points IMAX$\times{} $JMAX$\times{} $KMAX}} &
 \parbox{36pt}{\raggedright\multirow{2}{*}{\footnotesize Total Size}} &
 \multicolumn{6}{|l|}{\parbox{111pt}{\raggedright{\footnotesize Portioning of blocks}}} \\
\cline{5-10}
 &
 &
 &
 &
 \parbox{1pt}{\raggedright{\footnotesize I}} &
 \parbox{1pt}{\raggedright{\footnotesize J}} &
 \parbox{4pt}{\raggedright{\footnotesize K}} &
 \parbox{28pt}{\raggedright{\footnotesize \#Sub Blocks}} &
 \parbox{35pt}{\raggedright{\footnotesize Nodes / Processor}} &
 \parbox{39pt}{\raggedright{\footnotesize Processors}} \\
\hline
 \parbox{21pt}{\raggedright{\footnotesize 1}} &
 \parbox{72pt}{\raggedright{\footnotesize Boundary Layer}} &
 \parbox{60pt}{\raggedright{\footnotesize245$\times{}$70$\times{}$129}} &
 \parbox{36pt}{\raggedright{\footnotesize 2,212,350}} &
 \parbox{1pt}{\raggedright{\footnotesize 4}} &
 \parbox{1pt}{\raggedright{\footnotesize 2}} &
 \parbox{4pt}{\raggedright{\footnotesize 2}} &
 \parbox{28pt}{\raggedright{\footnotesize 16}} &
 \parbox{35pt}{\raggedright{\footnotesize 145,080}} &
 \parbox{39pt}{\raggedright{\footnotesize 1-16}} \\
\hline
 \parbox{21pt}{\raggedright{\footnotesize 2}} &
 \parbox{72pt}{\raggedright{\footnotesize Rudder body}} &
 \parbox{60pt}{\raggedright{\footnotesize114$\times{}$84$\times{}$84}} &
 \parbox{36pt}{\raggedright{\footnotesize 804,384}} &
 \parbox{1pt}{\raggedright{\footnotesize 3}} &
 \parbox{1pt}{\raggedright{\footnotesize 2}} &
 \parbox{4pt}{\raggedright{\footnotesize 1}} &
 \parbox{28pt}{\raggedright{\footnotesize 6}} &
 \parbox{35pt}{\raggedright{\footnotesize 140,868}} &
 \parbox{39pt}{\raggedright{\footnotesize 17-22}} \\
\hline
 \parbox{21pt}{\raggedright{\footnotesize 3}} &
 \parbox{72pt}{\raggedright{\footnotesize Rudder Cap}} &
 \parbox{60pt}{\raggedright{\footnotesize105$\times{}$74$\times{}$74}} &
 \parbox{36pt}{\raggedright{\footnotesize 574,980}} &
 \parbox{1pt}{\raggedright{\footnotesize 2}} &
 \parbox{1pt}{\raggedright{\footnotesize 2}} &
 \parbox{4pt}{\raggedright{\footnotesize 1}} &
 \parbox{28pt}{\raggedright{\footnotesize 4}} &
 \parbox{35pt}{\raggedright{\footnotesize 149,036}} &
 \parbox{39pt}{\raggedright{\footnotesize 23-36}} \\
\hline
 \parbox{21pt}{\raggedright{\footnotesize 4}} &
 \parbox{72pt}{\raggedright{\footnotesize Skeg}} &
 \parbox{60pt}{\raggedright{\footnotesize122$\times{}$64$\times{}$71}} &
 \parbox{36pt}{\raggedright{\footnotesize 554,368}} &
 \parbox{1pt}{\raggedright{\footnotesize 2}} &
 \parbox{1pt}{\raggedright{\footnotesize 1}} &
 \parbox{4pt}{\raggedright{\footnotesize 2}} &
 \parbox{28pt}{\raggedright{\footnotesize 4}} &
 \parbox{35pt}{\raggedright{\footnotesize 142,848}} &
 \parbox{39pt}{\raggedright{\footnotesize 27-30}} \\
\hline
 \parbox{21pt}{\raggedright{\footnotesize 5}} &
 \parbox{72pt}{\raggedright{\footnotesize Stabilizer body}} &
 \parbox{60pt}{\raggedright{\footnotesize89$\times{}$50$\times{}$64}} &
 \parbox{36pt}{\raggedright{\footnotesize 284,800}} & \parbox{1pt}{\raggedright{\footnotesize 2}} &
 \parbox{1pt}{\raggedright{\footnotesize 1}} &
 \parbox{4pt}{\raggedright{\footnotesize 1}} &
 \parbox{28pt}{\raggedright{\footnotesize 2}} &
 \parbox{35pt}{\raggedright{\footnotesize 144,000}} &
 \parbox{39pt}{\raggedright{\footnotesize 31-32}} \\
\hline
 \parbox{21pt}{\raggedright{\footnotesize 6}} &
 \parbox{72pt}{\raggedright{\footnotesize Stabilizer cap}} &
 \parbox{60pt}{\raggedright{\footnotesize92$\times{}$53$\times{}$58}} &
 \parbox{36pt}{\raggedright{\footnotesize 282,808}} &
 \parbox{1pt}{\raggedright{\footnotesize 2}} &
 \parbox{1pt}{\raggedright{\footnotesize 1}} &
 \parbox{4pt}{\raggedright{\footnotesize 1}} &
 \parbox{28pt}{\raggedright{\footnotesize 2}} &
 \parbox{35pt}{\raggedright{\footnotesize 144,478}} &
 \parbox{39pt}{\raggedright{\footnotesize 33-34}} \\
\hline
\end{tabular}
\end{center}
\vspace{2pt}
\caption {\label{tab:????}????}
\end{table}

